A second order finite volume IMEX Runge-Kutta scheme for two dimensional PDEs in finance

In this article we present a novel and general methodology for building second order finite volume implicit-explicit (IMEX) numerical schemes for solving two dimensional financial parabolic PDEs with mixed derivatives. In particular, applications to basket and Heston models are presented. The obtained numerical schemes have excellent properties and are able to overcome the well-documented difficulties related with numerical approximations in the financial literature. The methods achieve true second order convergence with non-regular initial conditions. Besides, the IMEX time integrator allows to overcome the tiny time-step induced by the diffusive term in the explicit schemes, also providing very accurate and non-oscillatory approximations of the Greeks. Finally, in order to assess all the aforementioned good properties of the developed numerical schemes, we compute extremely accurate semi-analytic solutions using multi-dimensional Fourier cosine expansions. A novel technique to truncate the Fourier series for basket options is presented and it is efficiently implemented using multi-GPUs.

==> subfigure/README <==
README
------

  The subfigure package has been superseded by the subfig package.
  The reason for the name change is that the new subfig package is not
  exactly backward compatible with this package; although, it comes
  with a configuration file that *almost* allows backward
  compatibility, the difference is that exact spacing and layout of
  the subfloats are not preserved.

  The newer (subfig) package is an improvement over this package and
  although this package will continue to be supported, it will no longer
  be updated.

This directory contains version 2.1.5 of the subfigure package.
Use `make' to extract the subfigure package and run the local tests.

MANIFEST:
---------
Makefile           UNIX makefile to extract the subfigure package
                       and related material.
README             This file.
subfigure.dtx      The documented subfigure package.
subfigure.ins      The subfigure package installation file.
subfigure.pdf      Subfigure package documentation (as PDF).
test.tex           Test one: Mixed tables and figures.
test2.tex          Test two: Check for extra space around figure
test3.tex          Test four: Test of optional args and \subref.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test for class \let of \endfigure, etc.

FILES AFTER `make':
-------------------
Makefile           UNIX makefile to extract the subfigure package
                       and related material.
README             This file.
ltxdoc.cfg         Configuration file to print change history and
                       index on the subfigure package documentation.       
subfigure.cfg      Set the preferred options for subfigure version 2.1.
subfigure.dtx      The documented subfigure package.
subfigure.ins      The subfigure package installation file.
subfigure.pdf      Subfigure package documentation (as PDF).
subfigure.ps       Subfigure package documentation (as PostScript).
subfigure.sty      The subfigure package 
test.ps            Results of test one.
test.tex           Test one: Mixed tables and figures.
test2.ps           Results of test two.
test2.tex          Test two: Check for extra space around figure
test3.ps           Results of test three.
test3.tex          Test four: Test of optional args and \subref.
test4.pdf          Results of test four.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test for class \let of \endfigure, etc.
test5a.ps          Results of test five (log file).
test5b.ps          Results of test five (output).

NOTES:
------

By default, the subfigure.sty file acts like the older versions of the
subfigure package.  To make the preferred options default move the
subfigure.cfg file into the standard TEXINPUTS path along with the
subfigure.sty file.  This reduces the whitespace around the subfigures
and subtables and sets the table style to have the captions and
subcaptions preceed the table and subtables.

